Project Dinos I: A joint lensing-dynamics constraint on the deviation from the power law in the mass profile of massive ellipticals

The mass distribution in massive elliptical galaxies encodes their evolutionary history, thus providing an avenue to constrain the baryonic astrophysics in their evolution. The power-law assumption for the radial mass profile in ellipticals has been sufficient to describe several observables to the noise level, including strong lensing and stellar dynamics. In this paper, we quantitatively constrained any deviation, or the lack thereof, from the power-law mass profile in massive ellipticals through joint lensing-dynamics analysis of a large statistical sample with 77 galaxy-galaxy lens systems. We performed an improved and uniform lens modelling of these systems from archival Hubble Space Telescope imaging using the automated lens modelling pipeline dolphin. We combined the lens model posteriors with the stellar dynamics to constrain the deviation from the power law after accounting for the line-of-sight lensing effects, a first for analyses on galaxy-galaxy lenses. We find that the Sloan Lens ACS Survey (SLACS) lens galaxies with a mean redshift of 0.2 are consistent with the power-law profile within 1.1$\sigma$ (2.8$\sigma$) and the Strong Lensing Legacy Survey (SL2S) lens galaxies with a mean redshift of 0.6 are consistent within 0.8$\sigma$ (2.1$\sigma$), for a spatially constant (Osipkov-Merritt) stellar anisotropy profile. We adopted the spatially constant anisotropy profile as our baseline choice based on previous dynamical observables of local ellipticals. However, spatially resolved stellar kinematics of lens galaxies are necessary to differentiate between the two anisotropy models. Future studies will use our lens models to constrain the mass distribution individually in the dark matter and baryonic components.

==> test.tex <==
\cyone{As discussed in Section \ref{Section4:Stellar_Kinematics}, we would need the anisotropy scale factor, $a_\text{ani}$, to estimate model-predicted stellar velocity dispersion, $\sigma_{\rm ap, PL }$ from our lens models and thus measure the mass-sheet transform parameter, $\lambda_{\rm int}$. We can however simultaneously obtain an estimate of mass-sheet transform parameter $\lambda_{\rm int}$ and the stellar anisotropy parameter, $a_\text{ani}$ with }\textsc{hierArc}\footnote{\url{https://github.com/sibirrer/hierArc}}, a software for Bayesian hierarchical analysis of strong lensing systems \citep{Birrer20}. Here, we provide a brief description of the Bayesian hierarchical framework. Let $D_i$ be the data for each \cyone{$i^{\rm th}$} individual lens and $D \equiv \{D_i\}_N$ be the dataset with all the data from $N$ number of lenses. \cyone{For this analysis, our individual lens data, $D_i$, consist of the lens model parameters such as the logarithmic slope, $\gamma_i$, and Einstein radius, $\theta_{{\rm E}, i}$ (used to obtain the power-law model-predicted stellar velocity dispersion, $\sigma_{{\rm ap, PL}, i}$), in addition to the measured velocity dispersion, $\sigma_{{\rm ap, meas}, i }$. For each $i^{\rm th}$ individual lens system, the individual lens parameter, $\xi_i$, is the  mass-sheet transform parameter $\lambda_{{\rm int}, i}$ and the stellar anisotropy parameter, $a_{{\rm ani}, i}$. For Bayesian hierarchical analysis, we sample the individual lens parameter, $\xi_i$ from a distribution parameterised by the population-level model parameters, $\Xi$. Using Bayer's theorem, we calculate the posterior of the population-level model parameters from the lensing dataset, $p(\Xi\mid D)$,}  by 
